A Survey of Adversarial Defenses in Vision-based Systems: Categorization, Methods and Challenges

Adversarial attacks have emerged as a major challenge to the trustworthy deployment of machine learning models, particularly in computer vision applications. These attacks have a varied level of potency and can be implemented in both white box and black box approaches. Practical attacks include methods to manipulate the physical world and enforce adversarial behaviour by the corresponding target neural network models. Multiple different approaches to mitigate different kinds of such attacks are available in the literature, each with their own advantages and limitations. In this survey, we present a comprehensive systematization of knowledge on adversarial defenses, focusing on two key computer vision tasks: image classification and object detection. We review the state-of-the-art adversarial defense techniques and categorize them for easier comparison. In addition, we provide a schematic representation of these categories within the context of the overall machine learning pipeline, facilitating clearer understanding and benchmarking of defenses. Furthermore, we map these defenses to the types of adversarial attacks and datasets where they are most effective, offering practical insights for researchers and practitioners. This study is necessary for understanding the scope of how the available defenses are able to address the adversarial threats, and their shortcomings as well, which is necessary for driving the research in this area in the most appropriate direction, with the aim of building trustworthy AI systems for regular practical use-cases.

==> bib.tex <==
@article{evasion,
  author    = {Battista Biggio and
               Igino Corona and
               Davide Maiorca and
               Blaine Nelson and
               Nedim Srndic and
               Pavel Laskov and
               Giorgio Giacinto and
               Fabio Roli},
  title     = {Evasion Attacks against Machine Learning at Test Time},
  journal   = {CoRR},
  volume    = {abs/1708.06131},
  year      = {2017},
  url       = {http://arxiv.org/abs/1708.06131},
  archivePrefix = {arXiv},
  eprint    = {1708.06131},
  timestamp = {Mon, 13 Aug 2018 16:48:20 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1708-06131},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{FSGM,
  title={Adversarial machine learning at scale},
  author={Kurakin, Alexey and Goodfellow, Ian and Bengio, Samy},
  journal={arXiv preprint arXiv:1611.01236},
  year={2016}
}
@article{MIFSGM,
  title={Boosting adversarial attacks with momentum},
  author={Dong, Yinpeng and Liao, Fangzhou and Pang, Tianyu and Su, Hang and Hu, Xiaolin and Li, Jianguo and Zhu, Jun},
  journal={arXiv preprint arXiv:1710.06081},
  year={2017}
}
@article{szegedy,
  title={Intriguing properties of neural networks},
  author={Szegedy, Christian and Zaremba, Wojciech and Sutskever, Ilya and Bruna, Joan and Erhan, Dumitru and Goodfellow, Ian and Fergus, Rob},
  journal={arXiv preprint arXiv:1312.6199},
  year={2013}
}
@article{basic,
  title={Making machine learning robust against adversarial inputs},
  author={Goodfellow, Ian and McDaniel, Patrick and Papernot, Nicolas},
  journal={Communications of the ACM},
  volume={61},
  number={7},
  pages={56--66},
  year={2018},
  publisher={ACM}
}
@article{papernot,
  title={Transferability in machine learning: from phenomena to black-box attacks using adversarial samples},
  author={Papernot, Nicolas and McDaniel, Patrick and Goodfellow, Ian},
  journal={arXiv preprint arXiv:1605.07277},
  year={2016}
}
@article{mnist,
  title={MNIST handwritten digit database},
  author={LeCun, Yann and Cortes, Corinna and Burges, CJ},
  journal={AT\&T Labs [Online]. Available: http://yann. lecun. com/exdb/mnist},
  volume={2},
  year={2010}
}
@article{cifar,
  title={The CIFAR-10 dataset},
  author={Krizhevsky, Alex and Nair, Vinod and Hinton, Geoffrey},
  journal={online: http://www. cs. toronto. edu/kriz/cifar. html},
  year={2014}
}
@inproceedings{imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={Computer Vision and Pattern Recognition, 2009. CVPR 2009. IEEE Conference on},
  pages={248--255},
  year={2009},
  organization={Ieee}
}
@article{sir_survey,
  author    = {Anirban Chakraborty and
               Manaar Alam and
               Vishal Dey and
               Anupam Chattopadhyay and
               Debdeep Mukhopadhyay},
  title     = {Adversarial Attacks and Defences: {A} Survey},
  journal   = {CoRR},
  volume    = {abs/1810.00069},
  year      = {2018},
  url       = {http://arxiv.org/abs/1810.00069},
  archivePrefix = {arXiv},
  eprint    = {1810.00069},
  timestamp = {Tue, 30 Oct 2018 10:49:09 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1810-00069},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{blackmarks,
  title={BlackMarks: Blackbox Multibit Watermarking for Deep Neural Networks},
  author={Chen, Huili and Rouhani, Bita Darvish and Koushanfar, Farinaz},
  journal={arXiv preprint arXiv:1904.00344},
  year={2019}
}
@article{deepmarks,
  title={DeepMarks: a digital fingerprinting framework for deep neural networks},
  author={Chen, Huili and Rohani, Bita Darvish and Koushanfar, Farinaz},
  journal={arXiv preprint arXiv:1804.03648},
  year={2018}
}
@article{deepsigns,
  title={DeepSigns: A Generic Watermarking Framework for Protecting the Ownership of Deep Learning Models},
  author={Rouhani, Bita Darvish and Chen, Huili and Koushanfar, Farinaz}
}
@article{dawn,
  title={Dawn: Dynamic adversarial watermarking of neural networks},
  author={Szyller, Sebastian and Atli, Buse Gul and Marchal, Samuel and Asokan, N},
  journal={arXiv preprint arXiv:1906.00830},
  year={2019}
}
@inproceedings{deepinspect,
  title={DeepInspect: A Black-box Trojan Detection and Mitigation Framework for Deep Neural Networks.},
  author={Chen, Huili and Fu, Cheng and Zhao, Jishen and Koushanfar, Farinaz},
  booktitle={IJCAI},
  pages={4658--4664},
  year={2019}
}
@article{tabor,
  title={Tabor: A highly accurate approach to inspecting and restoring trojan backdoors in ai systems},
  author={Guo, Wenbo and Wang, Lun and Xing, Xinyu and Du, Min and Song, Dawn},
  journal={arXiv preprint arXiv:1908.01763},
  year={2019}
}
@inproceedings{evasion,
  title={Evasion attacks against watermarking techniques found in mlaas systems},
  author={Hitaj, Dorjan and Hitaj, Briland and Mancini, Luigi V},
  booktitle={2019 Sixth International Conference on Software Defined Systems (SDS)},
  pages={55--63},
  year={2019},
  organization={IEEE}
}
@inproceedings{stealing,
  title={Stealing machine learning models via prediction apis},
  author={Tram{\`e}r, Florian and Zhang, Fan and Juels, Ari and Reiter, Michael K and Ristenpart, Thomas},
  booktitle={25th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 16)},
  pages={601--618},
  year={2016}
}
